A Newton-Based Method for Nonconvex Optimization with Fast Evasion of Saddle Points

Machine learning problems such as neural network training, tensor decomposition, and matrix factorization, require local minimization of a nonconvex function. This local minimization is challenged by the presence of saddle points, of which there can be many and from which descent methods may take inordinately large number of iterations to escape. This paper presents a second-order method that modifies the update of Newton's method by replacing the negative eigenvalues of the Hessian by their absolute values and uses a truncated version of the resulting matrix to account for the objective's curvature. The method is shown to escape saddles in at most $1 + \log_{3/2} (\delta/2\varepsilon)$ iterations where $\varepsilon$ is the target optimality and $\delta$ characterizes a point sufficiently far away from the saddle. This base of this exponential escape is $3/2$ independently of problem constants. Adding classical properties of Newton's method, the paper proves convergence to a local minimum with probability $1-p$ in $O\left(\log(1/p)) + O(\log(1/\varepsilon)\right)$ iterations.

==> ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi
%\usepackage{times}
% For figures
\usepackage{graphicx} % more modern
%\usepackage{epsfig} % less modern
%\usepackage{subfigure} 
\usepackage{float}


% For citations
%\usepackage{natbib}

% For algorithms
\usepackage{algorithm}
\usepackage{algorithmic}

% As of 2011, we use the hyperref package to produce hyperlinks in the
% resulting PDF.  If this breaks your system, please commend out the
% following usepackage line and replace \usepackage{icml2014} with
% \usepackage[nohyperref]{icml2014} above.
\usepackage{hyperref}

% Packages hyperref and algorithmic misbehave sometimes.  We can fix
% this with the following command.
%\newcommand{\theHalgorithm}{\arabic{algorithm}}

%\usepackage{ amsfonts, amsmath, amssymb, cite, verbatim, amsthm, comment}
%\usepackage{algorithm}
%\usepackage{algpseudocode}
%\usepackage{tikz}
%\usepackage{framed}
\usepackage{amsmath,amssymb}
%\usetikzlibrary{shapes,arrows}
%\input{figures/tikz_styles}
\usepackage{pgfplots}
\usepackage{color}
\input{my_sections.tex}
\usepackage{flushend}
\usepackage{multirow}
\usepackage{rotating}
\usepackage{appendix}
\usepackage{tikz,pgfplots}
\usepackage{subcaption}
\usepackage{bbm}



%\usetikzlibrary{matrix} % for block alignment
%\usetikzlibrary{arrows} % for arrow heads
%\usetikzlibrary{calc}   % for manimulation of coordinates
%\usetikzlibrary{shapes} % for ellipses and other shapes
\usepackage{standalone} % for standalone compilation
%\usetikzlibrary{positioning}
%\usetikzlibrary{backgrounds, fit}
%%\usepackage{graphics, subfigure, times, amsfonts, amsmath, amssymb, cite, verbatim, amsthm, comment}
%\usepackage{enumerate}
%\input{my_sections.tex}
%\usepackage{flushend}
%\usepackage{multirow}
%\usepackage{rotating}
%\input{mysymbol.sty}

% Shall we compile tike figures or not?
\newif\ifcompiletikz
\compiletikztrue





\input{mysymbol.sty}





%\usetikzlibrary{external} \tikzexternalize

%\addtolength{\textwidth}{20mm}
%\addtolength{\evensidemargin}{-2mm}
%\addtolength{\oddsidemargin}{-2mm}
%\addtolength{\textheight}{18mm} 
%\addtolength{\topmargin}{-0.9cm}

%
\newtheorem{assumption}{\hspace{0pt}\bf Assumption}
\newtheorem{comment}{\hspace{0pt}\bf Comment}
%\newtheorem{definition}{\hspace{0pt}\bf Definition}
%\newtheorem{lemma}{\hspace{0pt}\bf Lemma}
%\newtheorem{claim}{\hspace{0pt}\bf Claim}
%\newtheorem{proposition}{\hspace{0pt}\bf Proposition}
%\newtheorem{observation}{\hspace{0pt}\bf Observation}
%\newtheorem{theorem}{\hspace{0pt}\bf Theorem}
%\newtheorem{corollary}{\hspace{0pt}\bf Corollary}
%\newtheorem{fact}{\hspace{0pt}\bf Fact}
%\newtheorem{remark}{\hspace{0pt}\bf Remark}
%\newtheorem{test}{\hspace{0pt}\it Test Case}
%\newtheorem{definition}{\hspace{0pt}\bf Definition}
%
%\def \mlc {\text{\normalfont mlc}}
%\def \sep {\text{\normalfont sep}}
%\def \dom {\text{\normalfont dom}}
%\def\R {\text{\normalfont R}}
%\def\C {\text{\normalfont C}}
%\def\NR {\text{\normalfont NR}}
%\def\SR {\text{\normalfont SR}}
%\def\SL {\text{\normalfont SL}}
%\def\U {\text{\normalfont U}}
%\def\dis {\text{\normalfont dis}}








%strongly recommended
\numberwithin{theorem}{section}




% Declare title and authors, without \thanks
\newcommand{\TheTitle}{A Second Order Method for Nonconvex Optimization} 
\newcommand{\TheAuthors}{Santiago Paternain, Aryan Mokhtari, and Alejandro Ribeiro}

% Sets running headers as well as PDF title and authors
\headers{\TheTitle}{\TheAuthors}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{{\TheTitle}\thanks{Submitted to the editors DATE.
\funding{This work was funded by the Fog Research Institute under contract no.~FRI-454.}}}

% Authors: full names plus addresses.
\author{
  Santiago Paternain\thanks{University of Pennsylvania., Philadelphia, PA
    (\email{spater@seas.upenn.edu}, \url{http://www.seas.upenn.edu/\string~spater/}).}
  \and
  Aryan Mokhtari\thanks{University of Pennsylvania., Philadelphia, PA
    (\email{aryanm@seas.upenn.edu}, \url{http://www.seas.upenn.edu/\string~aryanm/}).}
  \and
  Alejandro Ribeiro\thanks{University of Pennsylvania., Philadelphia, PA
    (\email{aribeiro@seas.upenn.edu}, \url{http://www.seas.upenn.edu/\string~aribeiro/}).}
  \and
  Paul T. Frank\thanks{Department of Applied Mathematics, Fictional
    University, Boise, ID (\email{ptfrank@fictional.edu},
    \email{jesmith@fictional.edu}).}
  \and
  Jane E. Smith\footnotemark[3]
}
  }

\usepackage{amsopn}
%\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 


==> numerical.tex <==
%!TEX root = root.tex
\section{Numerical Experiments}\label{sec_numerical}
%
In this section we apply Algorithm \ref{alg_nonconvex_newton} to the matrix factorization problem, where the goal is to find a rank $r$ approximation of a given matrix $\bbM \in \ccalM^{l\times n}$. The problem can be written as
%
\begin{equation}
(\bbU^*,\bbV^*) := \argmin_{\bbU \in \ccalM^{l\times r}, \bbV \in \ccalM^{n\times r}}  f(\bbU,\bbV)=\argmin_{\bbU \in \ccalM^{l\times r}, \bbV \in \ccalM^{n\times r}}\frac{1}{2} \left\|\bbM-\bbU\bbV^{\top} \right\|_F^2.
\end{equation}
%
Writing the product $\bbU\bbV^{\top}$ as $\sum_{i=1}^r \bbu_i\bbv_i^{\top}$, where $\bbu_i$ and $\bbv_i$ are the $i$--th columns of the matrices $\bbU$ and $\bbV$ respectively. Let  $\bbx = [\bbu_1^{\top}, \ldots, \bbu_l^{\top}, \bbv_1^{\top}, \ldots \bbv_n^{\top}]^{\top}$, then we solve
%
\begin{equation}\label{eqn_application}
\bbx^* := \argmin_{\bbx \in \mathbf{R}^{r\times(n+l)}} f(\bbx).
\end{equation}
%
The matrix $\bbM \in \ccalM^{l\times n}$ is a rank one randomly generated matrix. We compare the performance of gradient descent and NCN (Algorithm \ref{alg_nonconvex_newton}) on the problem \eqref{eqn_application}. The step size in gradient descent is selected via line search by backtracking with parameters $\alpha$ and $\beta$ being the same as those of NCN. The parameters selected are $r=1$, $\alpha = 0.1$, $\beta=0.9$, accuracy $\varepsilon = 1\times10^{-12}$ and $m=\left\{1\times 10^{-3}, 1\times 10^{-12}\right\}$. The initial iterate selected for all simulations is the same and it is selected at random from a multivariate normal random variable with mean zero and standard deviation $100$. We star by considering an example where $n=l=10$, since in small problems the different behaviors of NCN for different values of $m$ are better illustrated. At the end of this section we consider an example with $n=l=100$ to show that the advantages of NCN over gradient descent are preserved in larger problems. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% F I G U R E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
        \includegraphics[width=\textwidth]{./figures/n_10_r1_m1e3.eps}
        %\caption{ }
        \label{fig_n_10_r_1_subopt}
    \end{subfigure}
%    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
      %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[b]{0.48\textwidth}
        \includegraphics[width=\textwidth]{./figures/n_10_r1_m1e3norm.eps}
        %\caption{ }
   \label{fig_n_10_r_1_grad}
    \end{subfigure}
    \vspace{-0.4cm}
    \caption{Comparison of gradient descent and NCN with $m = 1\times 10^{-3}$ in terms of suboptimality (left)  and norm of the gradient (right) for the rank on factorization problem. The dimension of the matrix to factorize is $10$ by $10$. }\label{fig_n_10_r_1m1e3}
\end{figure*}
%

In Figure \ref{fig_n_10_r_1m1e3} we plot suboptimality and the norm of the gradient in logarithmic scale for gradient descent and NCN with $m=1\times 10^{-3}$. After $500$ iterations the suboptimality achieved by NCN is $25$ orders smaller than that of gradient descent. In particular observe that gradient descent does not progress after $30$ iterations -- constant suboptimality -- since it is in the neighborhood of a saddlle -- norm of order $10^0$. On the contrary NCN succeeds in escaping this neighborhood efficiently. Indeed, after $30$ iterations approximately we observe an increase in the norm of the gradient, which illustrates the escape from the saddle. Moreover, in this region the decrease in the function value is smaller. In Figure \ref{fig_n_10_r_1m1e12} we present the results for NCN with $m=1\times 10^{-12}$. The conclusions of NCN in this case with gradient descent are the same as in the case with $m = 1\times 10^{-3}$.

Note however that the performance of NCN is affected by the different truncation level of the PT-inverse: the smaller $m$ is, the faster the  algorithm converges to the local minimum. Indeed, for $m = 1\times 10^{-3}$ the convergence rate is slower. Mainly due to the fact that it reaches a smaller neighborhood of the saddle point before avoiding it. Finally, for both levels of truncation of the PT-inverse, NCN --as well as gradient descent -- do not reach the neighborhood of the saddle point with $\left\| \nabla f(\bbx)\right\|<\varepsilon$, hence we do not add noise in NCN nor in gradient descent.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% F I G U R E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[t]
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
        \includegraphics[width=\textwidth]{./figures/n_10_r1m1e12subopt.eps}
        %\caption{ }
        \label{fig_n_10_r_1_suboptm}
    \end{subfigure}
%    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
      %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[b]{0.48\textwidth}
        \includegraphics[width=\textwidth]{./figures/n_10_r1_m1e12norm.eps}
        %\caption{ }
   \label{fig_n_10_r_1_gradm}
    \end{subfigure}
        \vspace{-0.4cm}
    \caption{Comparison of gradient descent and NCN with $m = 1\times 10^{-12}$ in terms of suboptimality (left)  and norm of the gradient (right) for the rank on factorization problem. The dimension of the matrix to factorize is $10$ by $10$. }\label{fig_n_10_r_1m1e12}
\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% F I G U R E %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[t]
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
        \includegraphics[width=\textwidth]{./figures/n_100_r1subopt.eps}
        %\caption{ }
        \label{fig_n_100_r_1_subopt}
    \end{subfigure}
%    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
      %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[b]{0.48\textwidth}
        \includegraphics[width=\textwidth]{./figures/n_100_r1grad.eps}
        %\caption{ }
   \label{fig_n_100_r_1_grad}
    \end{subfigure}
    \vspace{-0.4cm}
    \caption{Comparison of gradient descent and NCN with $m = 1\times 10^{-12}$ in terms of suboptimality (left)  and norm of the gradient (right) for the rank one factorization problem. The dimension of the matrix to factorize is $100$ by $100$. }\label{fig_n_100_r_1}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
In Figure \ref{fig_n_100_r_1} we depict the behavior of NCN and gradient descent where the matrix to factorize is $\bbM \in \ccalM^{100\times 100}$. As it can be observed in Figure \ref{fig_n_100_r_1} the comparative advantages of NCN over gradient descent in lower dimensions scale to high dimensions. This is while NCN escapes the saddle in $30$ iterations -- marked by the end of the plateau on the norm of the gradient of the function -- gradient descent stays in the neighborhood of the saddle point -- marked by the fact that the suboptimality is around $10^5$ and the norm of the gradient is $10^0$.   




